Flow Network Tracking for Spatiotemporal and Periodic Point Matching: Applied to Cardiac Motion Analysis

The accurate quantification of left ventricular (LV) deformation/strain shows significant promise for quantitatively assessing cardiac function for use in diagnosis and therapy planning (Jasaityte et al., 2013). However, accurate estimation of the displacement of myocardial tissue and hence LV strain has been challenging due to a variety of issues, including those related to deriving tracking tokens from images and following tissue locations over the entire cardiac cycle. In this work, we propose a point matching scheme where correspondences are modeled as flow through a graphical network. Myocardial surface points are set up as nodes in the network and edges define neighborhood relationships temporally. The novelty lies in the constraints that are imposed on the matching scheme, which render the correspondences one-to-one through the entire cardiac cycle, and not just two consecutive frames. The constraints also encourage motion to be cyclic, which is an important characteristic of LV motion. We validate our method by applying it to the estimation of quantitative LV displacement and strain estimation using 8 synthetic and 8 open-chested canine 4D echocardiographic image sequences, the latter with sonomicrometric crystals implanted on the LV wall. We were able to achieve excellent tracking accuracy on the synthetic dataset and observed a good correlation with crystal-based strains on the in-vivo data.

==> siamese_network.tex <==
% LEARNING
\subsection{Data driven feature generation and metric}
%
% MOTIAVATION
\subsubsection{Motivation} 
\par In any feature based tracking method, the quality of the tracking is highly dependent on the quality of the features. The features have to be both representative and discriminative. The features should capture underlying image statistic while at the same time also be unique and salient so different tissue classes, locations and orientations result in different features (if translational and rotational invariance is not desired). Similarly, the metric to calculate the distance between features is also of importance. We typically have no a-priori information regarding which feature component is important, and therefore should get weighed heavily.
%
\par For these reasons, we turn to learning based methods. This allows us to sidestep the tedious task of feature engineering and metric composition. We will explain how supervised, unsupervised and semi-supervised methods can be used and discuss the implications of each of these strategies. 
%
% SUPERVISED 
\subsubsection{Supervised method - Siamese Neural Network} From a set of simulated images and ground truth motion trajectories, we sampled pairs of similar image patches that are centered at consecutive points in the same trajectory and dissimilar image patches that are centered at points that are close but not in the same trajectory. Then we train a neural network to maximize representation distance between dissimilar patches and minimize it for similar patches. 
\par The network learns the weights $W$ that parametrize a function $G_W$ on the input signals (see Figure \ref{fig:siamese_network}), such that, $E_W(x_1, x_2) = ||G_W(x_1) - G_W(x_2))||$ is minimized when $x_1$ and $x_2$ are similar and maximized when they are dissimilar \cite{chopra2005learning} ($x_1$ is short for $I(x^t_i)$, the image patch centered at $x^t_1$ and similarly $x_2$ is short for $I(x^{t+1}_j)$).
%
\begin{figure}
	\centering
	\includegraphics[scale = .32]{images/siamese_network.png}		
	\caption{Siamese network: light gray - convolutional layer, dark gray - fully connected layer. ReLU activations used between layers. Input image patches are of size $11 \times 11 \times 11$.}
	\label{fig:siamese_network}
\end{figure}
%
%\par We used convolutional layers at the base of our network that learn features and a fully connected layer after the convolutional layers that learns how to weigh them in order to get a metric on the feature representations.
%
\par $y$, a binary label, is assigned to each pairs of patches $x_1$ and $x_2$. Similar pairs of patches are assigned the label $y = 1$ and dissimilar pairs are assigned $y = 0$. Learning is done by minimizing the following hinged contrastive loss function, which is more robust than a generic contrastive loss \cite{hadsell2006dimensionality}:
\begin{equation}
	L(W, y, x_1, x_2) = \frac{1}{2} y E_W^2 + \frac{1}{2} (1 - y) max(1- E_W, 0)^2 
\end{equation}
%
\par A test pair of image patches will result in a value $E_W \in [0, 1]$. For an edge $e^t_{ij}$ between $x^t_{i}$ and $x^{t+1}_{j}$, if we let the corresponding image patches be $I^t(x^t_{i})$ and $I^{t+1}(x^{t+1}_{j})$:
\begin{equation}
	E_W\left( x^t_{i}, x^{t+1}_{j}\right) = ||G_W\left(I^t(x^t_{i})
	\right) - G_W\left(I^{t+1}(x^{t+1}_{j})\right) ||
\end{equation}
%
\par This quantity is used to set edge weights on our flow network (see Equation \ref{eqn:edge_wt}). Key hyper-parameters, such as number of convolution kernels and the number of nodes in the fully connected layer were tuned via leave-one-out cross validation. Batch-normalization and dropout layers are used following all layers (except the final). Approximately $100,000$ patches were used for training.
%
%
% SEMI-SUPERVISED
\subsubsection{Transfer learning - using segmentation embedding}
%
It is rather difficult to collect labeled data of the nature we used to construct the Siamese neural network. There are no ground truth trajectories available for real life data. It is near impossible to manually mark where a image voxel has traversed across the cardiac cycle because of noise, inherent deformation and other uncertainties. Therefore, an unsupervised method can be of great value when no such labeled information is available. 
%
However, even though an unsupervised method might learn an embedding that best captures the variance of the data, the `axis' of these variations, might not be the most relevant for the task at hand. Therefore, we strike a compromise and train a neural network for the task of tissue segmentation with the hypothesis that this will allow us to learn a more discriminative embedding. Fig \ref{fig:semi_supervised_network} illustrates the design of such a network. 
%
\par Because the network is learning how to do semantic segmentation (and not just classification), it is also positionally aware of where the object is. Equation \ref{eqn:mahalanobis_wt} is used to calculate the distance between the learned representations. $F\left(x^t_{i}\right)$ represents the learned embedding on the image patch centered at $x^t_{i}$. $ C_f ^{-1}$ is the covariance matrix of the feature distances. 
\begin{equation}
\label{eqn:mahalanobis_wt}
	E_W\left( x^t_{i}, x^{t+1}_{j}\right) = \sqrt{F\left(x^t_{i}\right) C_f ^{-1} F\left(x^{t+1}_{j}\right)}
\end{equation}

\begin{figure}
	\centering
	\includegraphics[scale = .32]{images/semi_supervised_semantic_embedding.png}		
	\caption{Segmentation network: A low dimensional embedding of image patches, that captures images statistics but also positionally aware is learned.}
	\label{fig:semi_supervised_network}
\end{figure}
